Sequential Deliberation for Social Choice

In large scale collective decision making, social choice is a normative study of how one ought to design a protocol for reaching consensus. However, in instances where the underlying decision space is too large or complex for ordinal voting, standard voting methods of social choice may be impractical. How then can we design a mechanism - preferably decentralized, simple, scalable, and not requiring any special knowledge of the decision space - to reach consensus? We propose sequential deliberation as a natural solution to this problem. In this iterative method, successive pairs of agents bargain over the decision space using the previous decision as a disagreement alternative. We describe the general method and analyze the quality of its outcome when the space of preferences define a median graph. We show that sequential deliberation finds a 1.208- approximation to the optimal social cost on such graphs, coming very close to this value with only a small constant number of agents sampled from the population. We also show lower bounds on simpler classes of mechanisms to justify our design choices. We further show that sequential deliberation is ex-post Pareto efficient and has truthful reporting as an equilibrium of the induced extensive form game. We finally show that for general metric spaces, the second moment of of the distribution of social cost of the outcomes produced by sequential deliberation is also bounded.

==> discussion.tex <==
The simplest baseline algorithm against which to contrast deliberation is the random dictatorship: Choose an agent uniformly at random and use her preferred decision point.  It is not hard to see, following the analysis of Theorem~\ref{theorem:main}, that this procedure is a 2-approximation to the social welfare optimum.  Deliberation thus provides a meaningful improvement over the simple baseline.  Among the other advantages of deliberation, note that at no point do we need to elicit individual preferences in a cardinal or ordinal fashion; instead, we merely present an alternative proposal and ask two agents to bargain for their preferred decision point.  Indeed, it is not strictly necessary to characterize or even enumerate the entire decision space prior to deliberation, as would be necessary for a standard social choice procedure.  Also, it should be stressed that the \textit{procedure} of deliberation still makes sense if the decision space is not a median graph; only the analysis rests on this characterization.  Finally, though this advantage cannot be made precise, deliberation is a more participatory process than standard social choice or random dictatorship in that agents interact with one another and take part in a process of reaching consensus.  While it is beyond the scope of this work, it is not inconceivable that social and opinion dynamics during the process of deliberation actually improve the quality of discourse and the resulting outcome.  



==> lb.tex <==
\section{Random Dictatorship and the Second Moment} 
\label{sec:second}
A simple baseline algorithm for our problem is Random Dictatorship: Output the bliss point $p_u$ of a random agent $u \in \N$. Such an algorithm also satisfies the desiderata that we presented in Section~\ref{sec:properties}: The outcome is trivially Pareto-efficient and the mechanism is truthful.  Furthermore, the Distortion of random dictatorship on social cost is at most $2$, and Theorem~\ref{lb:random} shows this bound is tight. We now show three ways that sequential deliberation is much superior to Random Dictatorship despite their seeming similarity.  Proofs in this section are relegated to the appendix.

\subsection{Second Moment of Social Cost}
We first consider the second moment, or the expected squared social cost of sequential deliberation.  We study the Distortion on this metric. Recall that the {\em social cost} of an alternative $a \in \S$ is given by $ SC(a) = \sum_{u \in \N} d(p_u,a)$. Let $a^* \in \S$ be the minimizer of social cost, {\em i.e.}, the {\em generalized median}. Then define:
 $$ \mbox{Squared-Distortion} = \frac{\mathbb{E}[(SC(a))^2]}{(SC(a^*))^2}$$
 where the expectation is over the set of outcomes $a$ produced by Sequential Deliberation.  
  
We will first show that sequential deliberation has Squared-Distortion at most $3$. One way to interpret this result is that the deviation of the social cost around its mean falls off quadratically instead of linearly, which means the outcome of sequential deliberation is well-concentrated around its mean value. In contrast, we show that Random Dictatorship has unbounded Squared-Distortion. The motivation for considering Squared-Distortion instead of the standard deviation is that the latter might prefer a more deterministic mechanism with a worse social cost, a problem that the Squared-Distortion avoids.  

\begin{theorem}
\label{thm:squaredDistortion}
    For any median graph $\S$, the Squared-Distortion of sequential deliberation on $\S$ is at most $3$. Furthermore, the Squared-Distortion of random dictatorship is unbounded.
\end{theorem}
The proof of the theorem is given in appendix~\ref{app:thm:squaredDistortion}.


\subsection{Instance-wise Dominance in Social Cost} 
Even on the social cost metric (and not the squared value), we will now show something much stronger than what the worst-case Distortion bounds imply.

\begin{theorem}
\label{thm:random}
For any set of agents $\N$ and outcomes $\S$ that define a median graph, the expected social cost of sequential deliberation is at most that of random dictatorship.
\end{theorem}

The proof is in appendix~\ref{app:thm:random}. This shows that instance by instance, sequential deliberation does at least as well on the first moment of social cost as Random Dictatorship, and in addition, it has bounded second moment in the worst case, which Random Dictatorship does not have.

\subsection{Social Cost Under Near-Unanimity}
A final comparison between sequential deliberation and random dictatorship concerns the convergence to optimality under the ``easy case'' of nearly unanimous agents, i.e., when most agents have exactly the same bliss point.  The result for sequential deliberation is a simple corollary of Theorem~\ref{theorem:main} but is presented here for purpose of its comparison with random dictatorship. The proof is in appendix~\ref{app:cor:unanimous}.

\begin{definition}
    A set of agents $\N$ is said to be $\epsilon$-\textbf{unanimous} on a set of outcomes $\S$ if all but an $\epsilon$ fraction of the agents have the same bliss point in $\S$.
\end{definition}

\begin{corollary}
\label{cor:unanimous}
    Sequential deliberation with a $\epsilon$-unanimous set of agents $\N$ with bliss points on set $\S$ that defines a median graph has Distortion at most  $(1+\epsilon)$. In contrast, Random Dictatorship has Distortion $2 - \epsilon$.
\end{corollary}


%----------------------------------------------------%



